A Distanced Matching Game, Decremental APSP in Expanders, and Faster Deterministic Algorithms for Graph Cut Problems

Expander graphs play a central role in graph theory and algorithms. With a number of powerful algorithmic tools developed around them, such as the Cut-Matching game, expander pruning, expander decomposition, and algorithms for decremental All-Pairs Shortest Paths (APSP) in expanders, to name just a few, the use of expanders in the design of graph algorithms has become ubiquitous. Specific applications of interest to us are fast deterministic algorithms for cut problems in static graphs, and algorithms for dynamic distance-based graph problems, such as APSP. Unfortunately, the use of expanders in these settings incurs a number of drawbacks. For example, the best currently known algorithm for decremental APSP in constant-degree expanders can only achieve a $(\log n)^{O(1/\epsilon^2)}$-approximation with $n^{1+O(\epsilon)}$ total update time for any $\epsilon$. All currently known algorithms for the Cut Player in the Cut-Matching game are either randomized, or provide rather weak guarantees. This, in turn, leads to somewhat weak algorithmic guarantees for several central cut problems: for example, the best current almost linear time deterministic algorithm for Sparsest Cut can only achieve approximation factor $(\log n)^{\omega(1)}$. Lastly, when relying on expanders in distance-based problems, such as dynamic APSP, via current methods, it seems inevitable that one has to settle for approximation factors that are at least $\Omega(\log n)$. In this paper we propose the use of well-connected graphs, and introduce a new algorithmic toolkit for such graphs that, in a sense, mirrors the above mentioned algorithmic tools for expanders. One of these new tools is the Distanced Matching game, an analogue of the Cut-Matching game for well-connected graphs. We demonstrate the power of these new tools by obtaining better results for several of the problems mentioned above.

==> old-stuff.tex <==


\newpage
\section{Old Stuff}


\mynote{to check: a routing path may go through a terminal vertex. This does not create any problems? especially where we do path peelings?}


\begin{theorem}\label{thm: distancing or certificate}
	There is an algorithm that, given a graph $H$ on $N^{h-j}$ vertices, either computes a distancing $(A,B,E')$ of $H$ with $|A|=|B|\geq N^{h-j}/x_j$ and distance $\ell_j$, or certifies that for every pair $(X,Y)$ of disjoint subsets of vertices of $H$, with $|X|=|Y|\geq N^{h-j}/x'$, there is a collection $\qset$ of paths in $H$ connecting vertices of $X$ to vertices of $Y$, with length of every path $\ell'_j$ and congestion $\eta'_j$. The running time is $T(j)$.
\end{theorem} 

The remainder of this section is dedicated to the proof of the theorem.

\mynote{for now, throughout, will use parameters $d=32/\eps'$, and $d'=1024/(\eps'^2)$.  This gives $\Delta=64/\eps'$, so $d'=d\cdot \Delta$. Generally, will choose $\eps'$ to be something like $\eps^{10}$. So accumulation of factor that look like $N^{\poly(\eps')}$ are OK. At the end this will give us $N^{\poly(\eps')/\eps}<N^{\eps}$ as long as $\poly(\eps')<\eps^2$.}

\subsection{Base Case: Level-$(h-1)$ Graphs}

\begin{itemize}
	\item $d=32/\eps'$, $d'=1024/(\eps')^2$. This gives $\Delta=64/\eps'$, so $d'=d\cdot \Delta$.
	\item {\bf Certificate Case:} we compute partition $(U(H),(S(H))$ of $V(H)$.
	
	\begin{itemize}
		\item $|U(H)|\leq N^{1-\eps'}$.
		
		\item every pair $A,B$ of subsets of $S(H)$ of equal cardinality can be routed via paths of length at most $d'$, congestion $\eta'_{h-1}=N$. 
		\item $\Lambda_{h-1}=1$; the graph can only tolerate one edge deletion.
	\end{itemize}

\item {\bf Distancing Case:} distancing $(X,Y,E')$, where $E'=\emptyset$, $|X|=|Y|$ and $|X|\geq N^{1-2\eps'}$. Moreover, for every pair $x\in X,y\in Y$ of vertices, $\dist_G(x,y)\geq d$ holds.

\item Running time: $O(N^3)$.
\end{itemize}







\newpage
%----------------------------------

\subsection{Step: Level-$j$ Graph, for $j<h-1$}


\paragraph{Parameters.}
There are three different distance parameters.

\begin{itemize}
	\item $d=32/\eps'$ is the distance for all distancings. It needs to be large to ensure that the number of iterations in the distanced matching game is small.
	
	\item $d'=1024/(\eps')^2$ is the embedding length. Will also use $\Delta=64/\eps'$, so $d=d'\cdot \Delta$. We need it to be large because once we run out of embedding paths, we use \Cref{lem: find separation of terminals} to get the $d$-distancing. It requres that many terminals are at distance $d'$ from each other, and $\Delta$ should be sufficiently large.
	
	\item $d''_j$ is the distance value for the certificate. Will need to accumulate because we build on certificates of subgraphs, and their embeddings, to find the certificate for current graph.
\end{itemize}

\paragraph{Assumption:} there is an algorithm for level-$(j+1)$, that, in time $T_{j+1}$, does one of the following:
\begin{itemize}

	\item {\bf Certificate Case:}
	
	\begin{itemize}
		\item partitions $V(H)$ into $U(H)$ and $S(H)$, where $|U(H)|\leq \gamma_{j+1}\cdot |V(H)|=\gamma_{j+1}\cdot N^{h-j}$
		
		\item every pair $A,B$ of subsets of $S(H)$ can be routed via paths of length at most $d''_{j+1}$ in $H$, with congestion $\eta'_{j+1}$. 
		\item this graph can tolerate up to $\Lambda_{j+1}$ edge deletions.
	\end{itemize}
	
	\item {\bf Distancing Case:} distancing $(X,Y,E')$, where $|X|\geq |V(H)|/x_{j+1}$. Moreover, for every pair $x\in X,y\in Y$ of vertices, $\dist_G(x,y)\geq d$ holds.
\end{itemize}





\paragraph{End Result:} algorithm for level-$(j+1)$, that, in time $T_{j}=??$, does one of the following:
\begin{itemize}
	
	\item {\bf Certificate Case:}
	
	\begin{itemize}
		\item partitions $V(H)$ into $U(H)$ and $S(H)$, where $|U(H)|\leq \gamma_{j}\cdot |V(H)|=\gamma_{j}\cdot N^{h-j+1}$. Right now it looks like \highlightf{\gamma_j\geq \frac{2}{N^{\eps'}}+\gamma_{j+1}} is enough. Overall, $\gamma\leq 2/(N^{\eps'}\cdot \eps)$ will hold.
		
		\item every pair $A,B$ of subsets of $S(H)$ can be routed via paths of length at most $d''_{j}$ in $H$, congestion $\eta'_{j}$. 
		
		Final bound: can set $\eta'_h=N^5$, and $\eta'_j=\eta'_{j+1}\cdot N^{c\eps'/\eps^2}$. This will mean that $\eta'_0\leq N^{5+c\eps'/\eps^2}\leq N^6$ if $c\eps'<\eps^2$. Also $d''_j\leq 3d''_{j+1}\cdot d'$. So $d''_j$ is roughly $(2^{14}/\eps')^{h-j}$. Final bound will be $(2/\eps')^{O(1/\eps)}=2^{O(\log(1/\eps)/\eps)}\leq 2^{O(1/\eps^2)}$.
			
		\item this graph can tolerate up to $\Lambda_{j}$ edge deletions (how many vertices do we need to keep left in $S(H)$ to make it work?) \mynote{need: $\Lambda_j$ as function of $\Lambda_{j+1}$}
	\end{itemize}
	
	\item {\bf Distancing Case:} distancing $(X,Y,E')$, where $|X|\geq |V(H)|/x_{j}$. Moreover, for every pair $x\in X,y\in Y$ of vertices, $\dist_G(x,y)\geq d$ holds. \mynote{need: $x_j$ as functions of $x_{j+1}$}. From Stage 1: $x_j\geq N^{4\eps'/\eps}\cdot x_{j+1}$, and $x_j>N^{3\eps'}$. 
\end{itemize}


\paragraph{For later:} Embedding of level-$(j+1)$ graphs into $H$ has path length $d'$, congestion $\eta_j=N^{6\eps'/\eps}\cdot  (x_{j+1})^2$. Generally, $x_j\leq N^{O(\eps'/\eps^2)}$ will hold.

\newpage

\subsubsection{Stage 1: Subgraphs}
We assume that we are given a graph $H$ on $N^{h-j+1}$ vertices.
We partition the vertices of $H$ into $N$ subsets containing $N^{h-j}$ vertices each, $V_1,\ldots,V_N$. For all $1\leq i\leq N$, we construct a graph $H_i=(V_i,E_i)$, where initially $E_i=\emptyset$. Denote $\hset'=\set{H_1,\ldots,H_N}$. The stage is performed in iterations.

\subsubsection*{Iteration Description}
We apply the algorithm for level-$(j+1)$ to each current graph $H_1,\ldots,H_N$. We denote by $\hset_1\subseteq \hset$ the set of graphs $H_i$ for which the outcome is a distancing, and by $\hset_2\subseteq \hset$ the set of graphs for which the outcome is a certificate.

If $|\hset_1|\leq N^{1-\eps'}$, then we terminate Stage 1. The outcome is a subset $\hset_2\subseteq \hset$ of at least $N-N^{1-\eps'}$ graphs, and, for every graph $H_i\in \hset_2$, a partition $(S(H_i),U(H_i))$ of its vertices, such that the following hold:

\begin{itemize}
	\item $|U(H_i)|\leq \gamma_{j+1}\cdot |V(H_i)|=\gamma_{j+1}\cdot N^{h-j}$; and
	
	\item every pair $A,B$ of subsets of $S(H_i)$ can be routed inside $H_i$ via paths of length at most $d'$, and congestion $\eta'_{j+1}$. 
\end{itemize}

In the remainder of the description of the iteration, we assume that $|\hset^1|>N^{1-\eps'}$. Recall that, for every graph $H_i\in \hset^1$, we obtained a distancing $(X_i,Y_i,E'_i)$, where $|X_i|=|Y_i|\geq |V(H_i)|/x_{j+1}$, and $|E'_i|\leq |X_i|/16$.

\mynote{(want: matching of size $|X_i|/4$, then delete edges of $E'_i$.)}


Partition $\hset^1$ into classes $\hset^1_1,\ldots,\hset^1_z$, where $z\leq \log N$ \mynote{(assume that $x_{j+1}<N/2$)} Class $\hset^1_j$ contains all graphs $H_j$ with $\frac{N^{h-j}}{2^{j+1}}\leq |X_j|\leq \frac{N^{h-j}}{2^{j}}$. There is an index $j$ such that ${|\hset^2_j|\geq |\hset^1|/\log N\geq N^{1-\eps'}/\log N}$.


Start: $E^*=\emptyset$. For each $H_i\in \hset^1_j$, we greedily try to connect vertices of $X_i$ to vertices of $Y_i$ via paths of length $d'$, via path peeling. This takes time at most $|E(H)|\cdot d'$ per graph, at most $N\cdot |E(H)|\cdot d$ total.

Graph is successful if we found $|X_i|/4$ such paths, it is unsuccessful otherwise. Partition $\hset^1_j$ into two subsets, set $\gset^s$ of successful, and set $\gset^u$ of unsuccessful graphs.
Partition into two cases, depending whether $|\gset^s|\geq \alpha |\hset^2_j|$ or not holds. Assume first it does not hold.

Number of edges deleted so far (in $E^*$) is at most $|\gset^s|\cdot \frac{N^{h-j}}{2^{j}}\cdot d'\leq \alpha\cdot |\hset^2|\cdot \frac{N^{h-j}}{2^{j}}\cdot d'$. Want to know which $\alpha$ is OK to use.


Let's look at the graphs in $\gset^u$. For each such graph $H_i$, we denote by $X'_i\subseteq X_i$, $Y'_i\subseteq Y_i$ the sets of vertices that are not routed yet. Because $H_i$ is unsuccessful, $|X'_i|=|Y'_i|\geq |X_i|/2\geq \frac{N^{h-j}}{2^{j+2}}$. Also, $\dist_{H\setminus E^*}(X'_i,Y'_i)\geq d'$. Denote $T=\bigcup_{H_i\in \gset^u}(X'_i\cup Y'_i)$. Then: 

$$|T|\geq |\gset^u|\cdot \frac{N^{h-j}}{2^{j+1}}\geq |\hset_j^2|\cdot \frac{N^{h-j}}{2^{j+2}}\geq N^{1-\eps'}\cdot \frac{N^{h-j}}{2^{j+2}\cdot \log N}$$

Consider now some terminal $t\in T$, and assume that $t\in X_i$, for some $H_i\in \gset^u$. Consider $B=B_{H\setminus E^*}(t,d'/2)$. Note that for all $H_a\in \gset^u$, $\dist_{H\setminus E^*}(X'_a,Y'_a)\geq d'$. So $B$ may not contain a vertex of $X'_a$ and a vertex of $Y'_a$. Therefore, $|B\cap T|\leq |T|/2$.

We apply \Cref{lem: find separation of terminals} to graph $G=H\setminus E^*$, the set $T$ of terminals, and sitance parameters $d$ and $\Delta'$. Note that, from the above discussion, for every terminal $t\in T$, there are at most $|T|/2$ terminals in $B_G(t,\Delta\cdot d/2)=B_G(t,d'/2)$. The algorithm then computes 
two subsets $(T_1,T_2)$ of terminals, with $|T_1|=|T_2|$, such that $|T_1|\geq \frac{|T|}{4|V(H)|^{32/\Delta}}$, and for every pair $t\in T_1$, $t'\in T_2$ of terminals, $\dist_G(t,t')\geq d$. 
The running time of the algorithm is $O(|E(H)|\cdot |V(H)|^{32/\Delta})$.


Note that:

\[
\begin{split}
|T_1|&\geq \frac{|T|}{4|V(H)|^{32/\Delta}}\\
&\geq \frac{N^{1-\eps'}\cdot N^{h-j}}{2^{j+1}\cdot \log N}\\
&\geq \frac{|V(H)|}{N^{\eps'}\cdot 4|V(H)|^{32/\Delta}\cdot 2^{j+2}\cdot \log N}\\
&\geq \frac{|V(H)|}{N^{4\eps'/\eps}\cdot 2^{j}}\\
&\geq \frac{|V(H)|}{N^{4\eps'/\eps}\cdot x_{j+1}}
\end{split}
\]

At the same time:


\[
\begin{split}
|E^*|&\leq \alpha\cdot |\hset^2|\cdot \frac{N^{h-j}}{2^{j}}\cdot d'\\
&\leq \alpha\cdot\frac{|V(H)|\cdot d'}{2^j}
\end{split}
\]

If we ensure that \highlightf{\alpha<\frac{1}{N^{4\eps'/\eps}\cdot x_{j+1}\cdot d'}}, then we obtain a valid distancing. In this distancing, \highlightf{x_j\geq N^{4\eps'/\eps}\cdot x_{j+1}} must hold.



Now consider Case 2, where $|\gset^s|\geq \alpha |\hset^1_j|$. We found matchings for at least $\alpha \cdot |\hset^2_j|$ graphs, that is:

\[
\begin{split}
|\gset^s|&\geq \alpha \cdot |\hset^1_j|\\
&\geq \frac{1}{N^{4\eps'/\eps}\cdot x_{j+1}\cdot d'}\cdot \frac{|\hset^1|}{\log N}\\
&\geq  \frac{1}{N^{4\eps'/\eps}\cdot x_{j+1}\cdot d'}\cdot \frac{N^{1-\eps'}}{\log N}\\
&\geq \frac{N}{N^{5\eps'/\eps}\cdot x_{j+1}}
\end{split}
\]



If we take a single level-$(j+1)$ graph $H'$, then its distancing parameters are: $|V(H')|/x_{j+1}$ and $d$. From \Cref{claim: distancing-matching game}, 
the number of iterations in which we can add matchings to a level-$(j+1)$ graph is at most:

$$\frac{32|V(H')|^{1+4/d}}{|V(H')|/x_{j+1}}\leq |V(H')|^{4/d}\cdot x_{j+1}=N^{\eps'(h-j)/8}\cdot x_{j+1}$$

because $d=32/\eps'$ and $|V(H')|=N^{h-j}$.
So total number of matchings we could be adding to the level-$(j+1)$ graphs is at most $N\cdot N^{\eps'(h-j)/8}\cdot x_{j+1}$. In every iteration, we add matchings to  $\frac{N}{N^{5\eps'/\eps}\cdot x_{j+1}}$ graphs. So total number of iterations is bounded by:

\[ N^{5\eps'/\eps}\cdot N^{\eps'(h-j)/8}\cdot (x_{j+1})^2  \leq N^{6\eps'/\eps}\cdot  (x_{j+1})^2 \]

because $h=1/\eps$. This is the congestion of the embedding, $\eta_j=N^{6\eps'/\eps}\cdot  (x_{j+1})^2$. Assuming that $x_j$ grows as before, we can assume that $x_j\leq N^{O(\eps'/\eps^2)}$ always holds. So generally the number of iterations is bounded by $N^{O(\eps'/\eps^2)}$. This means that in every graph that we get, $|E(H)|\leq |V(H)|\cdot N^{O(\eps'/\eps^2)}$.


\subsection*{Running Time Analysis of Phase 1.}

\paragraph{Analysis of an Iteration}
First, we apply the level-$(j+1)$ algorithm $N$ times. This gives run time $N\cdot T_{j+1}$.

Path Peeling: done at most $N$ times, runtime for each at most $|E(H)|\cdot N\cdot d'$.
Overall, if iteration is successful, its running time at most $|E(H)|\cdot N\cdot d'+N\cdot T_{j+1}$. Number of successful iterations is bounded by 
$N^{6\eps'/\eps}\cdot  (x_{j+1})^2$.

Run time of \Cref{lem: find separation of terminals} is $O(|E(H)|\cdot |V(H)|^{32/\Delta})=O(|E(H)|\cdot |V(H)|^{\eps'/2})$.

Total running time of Phase 1 is bounded by:


\[(|E(H)|\cdot N\cdot d'+N\cdot T_{j+1})\cdot N^{6\eps'/\eps}\cdot  (x_{j+1})^2+  O(|E(H)|\cdot |V(H)|^{\eps'/2}). \]


Rough estimate: $T_j\leq T_{j+1}\cdot N^{1+O(\eps'/\eps^2)}$. This would mean that $N_0\leq N^{h+O(\eps'/\eps^3)}\cdot T_{h-1}$, which is good.



\newpage
@@@@@@@@@=================


\subsection{Certification of the Certificate}

Remains to show:

\begin{lemma}\label{lem: certificate correct}
Suppose the algorithm ended with a certificate. Then for every pair $(A,B)$ of equal-cardinality subsets of $S(H)$, there is a collection of paths in $H$, of length at most $d''$ each, routing every vertex of $A$ to a distinct vertex of $B$, with congestion at most $\eta'_j$.
\end{lemma}

In the remainder of this subection, we prove the above lemma.
Denote by $\hset^*\subseteq \hset_2$ the set of good graphs. From \Cref{obs: many good graphs}, $|\hset^*|\geq N-2N^{1-\eps'}$. For each good graph $H_i\in \hset^*$, we are given a set $S(H_i)$ of at least $(1-\gamma_{j+1})\cdot N^{h-j}$ supported vertices.
Recall that $S(H)\subseteq \bigcup_{H_i\in \hset^*}S(H_i)$.

Let $(A,B)$ be two equal-cardinality sets of vertices in $H$.


\mynote{don't need this claim for now.}
\begin{claim}\label{claim short-path flow to paths}
Let $G$ be a graph, $S,T$ two subsets of its vertices, and $\pset(S,T)$ the set of all paths in $G$ connecting a vertex of $S$ to a vertex of $T$, such that the length of the path is at most $d$. Suppose there is a flow $f$ in $G$, defined over the set $\pset(S,T)$ of paths, in which every vertex of $S$ sends one flow unit, every vertex of $T$ receives one flow unit, and the congestion of the flow is $\eta$. Then there is a collection $\qset(S,T)$ of paths in $G$, such that the length of every path is at most $d$, and the paths route every vertex of $S$ to a distinct vertex of $T$, with congestion at most $d\cdot \eta$.
\end{claim}

\begin{proof}
	Sketch: we build a directed layered graph, with $d$ layers. For every layer contains all vertices of $G$. Every pair $L_i,L_{i+1}$ of layers, 
	for every edge $e=(u,v)\in E$, we add an edge $(x(u,i),x(v,i+1))$, and an edge $(x(v,i),x(u,i+1))$ of capacity $\eta$. We also add an edge $(x(u,i),x(u,i+1))$ of capacity $\infty$. Then we add a source $s$ that connects to every vertex $x(v,1)$ for $v\in S$, with capacity-$1$ edge, and destination $t$, to which every vertex $x(v,d)$ with $v\in T$ connects. Flow $F$ naturally defines an $s$-$t$ flow of value $|S|$ with no congestion in this network. Can use integrality of flow to get integral flow. This set of paths can be transformed into the desired set $\qset(S,T)$ of paths in graph $G$ by contracting all edges of infinite capacity. Because every edge of $G$ has $d$ copies in the flow network, new congestion will be $\eta\cdot d$.
\end{proof}

Let $\pset(A,B)$ be the set of all flow-paths connecting vertices of $A$ to vertices of $B$, whose length is at most $2d''_{j+1}+d'$. We construct a flow $F$ over paths in $\pset(A,B)$, where every vertex of $A$ sends one flow unit, every vertex of $B$ receives one flow unit, and the congestion is at most $\eta_{j+1}'$.

We do this in three steps.


\subsection*{Step 1}
Process each $H_i\in \hset^*$ one by one. When $H_i$ is processed, denote $N^A_i=|A\cap S(H_i)|$ and $N^B_i=|V\cap S(H_i)|$. Denote $\beta_i=\min\set{N^A_i,N^B_i}$.

Select arbitrary subset $S'_i\subseteq A\cap S(H_i)$ of cardinality $\beta_i$, and arbitrary subset $T'_i\subseteq B\cap S(H_i)$ of cardinality $\beta_i$. Recursive certificate property gives us a set $\pset'_i$ of paths in graph $H_i$, routing every vertex of $S'_i$ to a distinct vertex of $T'_i$ via paths of length at most $d''_{j+1}$, and with congestion $\eta'_{j+1}$. We use the embedding of all graphs in $\hset^*$ into $H$ with congestion \highlightf{\eta_j=N^{6\eps'/\eps}\cdot (x_{j+1})^2} (generally, $x_j\leq N^{O(\eps'/\eps^2)}$) via paths of length at most $d'$ to route all vertices in $\bigcup_{H_i\in \hset^*}S'_i$ to vertices of $\bigcup_{H_i\in \hset^*}T'_i$ in graph $H$. This routing causes congestion at most:
 
 \highlightf{\eta'_{j+1}\cdot \eta_j\leq \eta'_{j+1}\cdot N^{6\eps'/\eps}\cdot (x_{j+1})^2} 
 
 
 (so roughly speaking, $\eta'_{j}\leq \eta'_{j+1}\cdot N^{O(\eps'/\eps)}$ for now)
 
 and the length of the paths is at most: \highlightf{d'\cdot d''_j}.

\mynote{final APSP path length will be $2^{1/\poly(\eps)}$}


We partition the remaining graphs of $\hset^*$ into three subsets. Set $\hset^N$ contains all graphs $H_i$ in which $N_i^A=N_i^B$. We no longe need to route any vertices in such graphs. Set $\hset^A$ contains graphs $H_i\in \hset^*$ with $N_i^A>N_i^B$. For each such graph $H_i$, we denote by $D(H_i)=N_i^A-N_i^B$, and by $R_i=( A \cap S(H_i))\setminus S'_i$ the set of vertices that remains to be routed. Cleraly, $|R_i|=D(H_i)$. Similarly, set $\hset^B$ contains graphs 
 $H_i\in \hset^*$ with $N_i^B>N_i^A$. For each such graph $H_i$, we denote by $D(H_i)=N_i^B-N_i^A$, and by $R_i=( B \cap S(H_i))\setminus S'_i$ the set of vertices that remains to be routed. As before, $|R_i|=D(H_i)$ holds. Notice also that, since $|A|=|B|$, $\sum_{H_i\in \hset^A}D(H_i)=\sum_{H_i\in \hset^B}D(H_i)$ must hold.  Denote $\hat A=\bigcup_{H_i\in \hset_A}R_i$ and $\hat B=\bigcup_{H_i\in \hset_B}R_i$. 
 Let $\hat \pset$ be the set of all paths $\hat P$ in graph $H$, such that $\hat P$ originates at a vertex of $\hat A$, terminates at a vertex of $\hat B$, and has length at most $d''_j$.
 It is now enough to prove the following lemma.
 
 
 \mynote{don't need flow, we actually find the paths}
 \begin{lemma}\label{lem: good routing}
 	There is a flow $\hat f$ in graph $H$, defined over the paths in $\hat P$, such that every vertex of $\hat A$ sends exactly one flow unit, every vertex of $\hat B$ receives exactly one flow unit, and the congestion of the flow is at most $\eta'_{j+1}$.
 	\end{lemma}
 
Complete the proof of \Cref{lem: certificate correct} using \Cref{lem: good routing}...



From now on we focus on the proof of \Cref{lem: good routing}.

\mynote{vertices of $\hat G$ should be called nodes, edges super-edges, to distinguish between them and vertices/edges of $H$.}

\subsection*{Step 2: Star-Cover Structure} 
Will use star-cover and recursive properties of level-$(j+1)$ construction. 
Intuitively, we will define a bipartite graph $\hat G=(X,Y,E')$, with vertices of $X$ representing graphs of $\hset^A$, and vertices of $Y$ representing graphs of $\hset^B$, that is, 
$X=\set{v_i\mid H_i\in \hset_A}$ and $Y=\set{v_i\mid H_i\in \hset_B}$. We place an edge $e=(v_i,u_j)$ in the graph, with weight $w(e)$, to signify that we will send $w(e)$ flow units between vertices of $R_i$ and vertices of $R_j$. We will then require that, for every vertex $v_i\in V(\hat G)$, the total weight of all edges incident to $v_i$ in $\hat G$ is exactly $D(H_i)$. In order to be able to construct the required flow efficiently, we will decompose graph $\hat G$ into a collection of star graphs, where every vertex of $\hat G$ only participates in a constant number of the star graphs. Using this star-covering structure we will then construct the required flow. We now define the star-cover structure.

\begin{definition}[Star-Cover Structure]
A star-cover structure consists of:

\begin{itemize}
	\item A bipartite graph $\hat G=(X,Y,E')$, where $X=\set{v_i\mid H_i\in \hset_A}$ and $Y=\set{v_i\mid H_i\in \hset_B}$;
	
	\item For every edge $e\in E'$, an integral weight $w(e)\geq 0$, such that for every vertex $v_i\in V(J)$, $\sum_{e\in \delta_{\hat G}(v_i)}w(e)=D(H_i)$;
	
	\item A collection $\jset$ of star graphs, for which the following hold:
	
	\begin{itemize}
		\item each star graph $J\in \jset$ is a subgraph of $\hat G$;
		\item every edge of $\hat G$ participates in exactly one star; and
		\item every vertex of $\hat G$ participates in at most $2$ stars in $\jset$.
\end{itemize}
\end{itemize}
\end{definition}


\begin{claim}\label{claim: star cover structure}
	There is an efficient algorithm for computing a star-cover structure.
\end{claim}
\begin{proof}
	For convenience, we denote $\hset^A=\set{H_1,H_2,\ldots,H_r}$, and for all $1\leq i\leq r$, we denote $D(H_i)$ by $D_i$. We assume that the graphs are indexed so that $D_1\geq D_2\geq\cdots\geq D_r$. We also denote $\hset^B=\set{H'_1,H'_2,\ldots,H'_{r'}}$, and for $1\leq i\leq r'$, we denote $D(H'_i)$ by $D'_i$. We assume that the graphs are indexed so that $D'_{1}\leq D'_2\leq\cdots\leq D'_{r'}$. 
	
	We start with graph $\hat G$ containing the set $X\cup Y$ of vertices, where $X=\set{v_1,\ldots,v_r}$, with vertex $v_i$ representing graph $H_i$, and $Y=\set{v'_1,\ldots,v'_{r'}}$, with vertex $v'_i$ represeinting graph $H_i$. Initially, the graph contains no edges, and the set $\jset$ of stars is empty. We will then gradually add starts to $\jset$, and their corresponding edges to graph $\hat G$.
		
		
Let $D=\sum_{j=1}^rD_i=\sum_{j'=1}^{r'}D'_{j'}$. Consider the interval $I=(0,D]$. We consider two partitions of this interval.

The first partition, $\Pi$ is into consecutive intervals of lengths $D_1,D_2,\ldots,D_r$ in this order. In other words, we let $p_0=0$, $p_r=D$, and for $1\leq j<r$, we let $p_j=\sum_{a=1}^jD_a$. We denote the resulting set of intervals by $\iset=\set{I_1,I_2,\ldots,I_r}$, where for all $1\leq j\leq r$, $I_j=(p_{j-1},p_j]$.

The second partition, $\Pi'$,  is into consecutive intervals of lengths $D'_1,D'_2,\ldots,D'_{r'}$ in this order. In other words, we let $p'_0=0$, $p'_{r'}=D$, and for $1\leq j<{r'}$, we let $p_j=\sum_{a=1}^jD'_a$. We denote the resulting set of intervals by $\iset'=\set{I'_1,I'_2,\ldots,I'_{r'}}$, where for all $1\leq j\leq r'$, $I'_j=(p'_{j-1},p'_j]$.
Note that the lengths of the intervals in $\iset$ are non-increasing with their indices, while the lengths of the intervals in $\iset'$ are non-decreasing with their indices.

Let $j^*$ be the smallest index, such that $I_{j^*}$ is strictly contained in some interval of $\iset'$; denote this interval by $I'_{j^{**}}$. Clearly, none of the intervals of $\set{I_1,I_2,\ldots,I_{j^*-1}}$ is strictly contained in an interval of $\iset'$. Moreover, the length of $I_{j^*}$ must be less than the length of $I'_{j^{**}}$. Therefore, none of the intervals in $\set{I'_{j^{**}}, I'_{j^{**}+1}, I'_{r'}}$ may be contained in an interval of $\iset$.


For all $1\leq a\leq j^*-1$, we construct a star $J_a$, whose center vertex is $v_a$. For every interval $I'_{a'}$ that is contained in $I_a$, we add an edge $(v_a,v'_{a'})$ to the star $J_a$, whose weight is $D'_{a'}$ (the length of interval $I'_{a'}$). If an interval $I'_{a''}$ has a non-empty intersection with $I_a$, but is not contained in $I_a$, then we add an edge  $(v_a,v'_{a''})$ to the star $J_a$, whose weight is the length of the intersection of $I_a$ and $I'_{a''}$. Note that the sum of weights of all edges in star $J_a$ is precisely the length of the interval $I_a$, which is exactly $D_a$. For every index $1\leq j<j^*$, vertex $v_j$ serves as a center of exactly one star. For every index $1\leq j'<j^{**}$, vertex $v'_{j'}$ may serve as a leaf of at most two stars. In this case, the sum of weights of the two edges that are incident to $v'_{j'}$ in these stars is precisely the length of the interval $I'_{j'}$, which is equal to $D'_{j'}$. Lastly, vertex $v'_{j^{**}}$ may serve as a leaf of at most one star.

For all $j^{**}<a'\leq r'$, we consruct a star  $J'_{a'}$, whose center vertex is $v'_{a'}$. For every interval $I_{a}$ that is contained in $I'_{a'}$, we add an edge $(v'_{a'},v_{a})$ to the star $J'_{a'}$, whose weight is $D_{a}$ (the length of interval $I_{a}$). If an interval $I_{a''}$ has a non-empty intersection with $I'_{a'}$, but is not contained in $I'_{a'}$, then we add an edge  $(v'_{a'},v_{a''})$ to the star $J'_{a'}$, whose weight is the length of the intersection of $I'_{a'}$ and $I_{a''}$. Note that the sum of weights of all edges in star $J'_{a'}$ is precisely the length of the interval $I'_{a'}$, which is exactly $D'_{a'}$. For every index $j^{**}<a'\leq r'$, vertex $v'_{a'}$ serves as a center of exactly one star. For every index $j^*+1\leq a\leq r$, vertex $v'{a}$ may serve as a leaf of at most two stars. In this case, the sum of weights of the two edges that are incident to $v_{a}$ in these stars is precisely the length of the interval $I_{a}$, which is equal to $D_{a}$. 

Finally, we add another star $J^*$, whose center vertex is $v'_{j^{**}}$. 
Recall that interval $I_{j^*}$ is contained in interval $I'_{j^{**}}$. The subinterval of $I'_{j^{**}}$ between its first endpoint $p'_{j^{**}-1}$ and the left endpoint $p_{j^*-1}$ of $I_{j^*}$ was already included in the construction of the star $J_{j^*-1}$. Therefore, we let $I^*\subseteq I'_{j^{**}}$ be the subinterval of $I'_{j^{**}}$ between $p_{j^*-1}$ and $p'_{j^{**}}$. We think of the center of the star  $J^*$ as being associated with the interval $I^*$. In other words,  for every index $1\leq a\leq r$, if interval $I_a$ has a non-empty intersection with $I^*$, then we add an edge $(v'_{j^{**}}, v_a)$ to star $J^*$, whose weight is the length of the intersection of $I^*$ and $I_a$.
(we note that vertices $v'_{j^{**}}$ and $v_{j^*}$ are the only vertices that may serve both as a center of one star and as a leaf of another star).


To summarize, we have obtained a collection $\jset$ of stars. We can associate, with each star $J\in \jset$, a subinterval $I(J)\subseteq (0,D]$: if $J=J^*$, then $I(J)=I^*$; otherwise it is the interval of $\iset$ or of $\iset'$ that is associated with the center of the star. The intervals of $\set{I(J)\mid J\in \jset}$ partition the interval $(0,D]$.
\end{proof}






\subsection*{Step 3: Global Routing}

Consider some edge $e=(v_i,v'_j)\in \hat G$. From \Cref{obs: good graphs can route}, there exists a set $\pset(v_i,v'_j)$ of paths in graph $H$, such that:

\begin{itemize}
	\item Every path in $\pset(v_i,v'_j)$ originates at a vertex of $S(H_i)$ and terminates at a vertex of $S'(H_j)$; every vertex of $S(H_i)\cup S(H'_j)$ is an endpoint of at most one such path;
	\item $|\pset(v_i,v'_j)|=\ceil{7N^{h-j}/8}$;
	\item paths in $\pset(v_i,v'_j)$ cause congestion at most $N^3$ in $H$, and each path has length at most $d'$.
\end{itemize}

We denote by $M_{i,j}$ the matching that is defined by the paths of $\pset(v_i,v'_j)$, that is, $(x,y)\in M_{i,j}$ if and only if there is  a path $P(x,y)\in \pset(v_i,v'_j)$ whose endpoitns are $x$ and $y$. Clearly, $|M_{i,j}|=\ceil{7N^{h-j}/8}$. Notice that $w(e)\leq N^{h-j}$ must hold. We will select, for every edge $e=(v_i,v'_j)\in \hat G$, a multi-set $M'_{i,j}$ of pairs $(x,y)\in M_{i,j}$, of cardinality $w(e)$. We will ensure that, for every vertex $v_i\in X$, a vertex $x\in S(H_i)$ participates in at most two pairs in $\bigcup_{e=(v_i,v'_j)\in \delta_{\hat G}(v_i)}M'_{i,j}$, and the same holds for vertices of $Y$. For every edge $e=(v_i,v'_j)\in \hat G$, we will then use paths $P(x,y)\in \pset(v_i,v'_j)$ for pairs $(x,y)\in M'_{i,j}$ for \emph{exteran routing}. Let $\pset'$ denote the resulting collection of all such paths. For every graph $H'\in \hset^A\cap \hset^B$, for every vertex $x\in S(H')$, we denote by $k(x)\in \set{0,1,2}$ the number of paths in $\pset'$, for which $x$ serves as an endpoint. Our construction guarantees that $\sum_{x\in S(H')}k(x)=D(H')$. In our last step, we perform \emph{local routing}, in which, for every graph $H'\in \hset^A\cup \hset^B$, we connect every vertex of $R(H')$ to some other vertex of $S(H')$, such that every vertex $x\in S(H')$ has exactly $k(x)$ paths teminating at it. This local routing explores the certificate properties of the graphs in $\hset$, and the embedding of these graphs into $H$.

We now state the following lemma that allows us to perform a global routing.

\begin{lemma}\label{lem: global}
	For every edge $e=(v_i,v'_j)\in E(\hat G)$, there is a multiset $M'_{i,j}\subseteq M_{i,j}$ of pairs of vertices of cardinality $w(e)$. For every graph $H_i\in \hset^A$ and vertex $x\in S(H_i)$, let $k(x)$ be the total number of pairs in $\bigcup_{e=(v_i,v'_j)\in \delta_{\hat G}(v_i)}M'_{i,j}$, in which vertex $x$ participates. Then $\sum_{x\in S(H_i)}k(x)=D(H_i)$, and for every vertex $x\in S(H_i)$, $k(x)\in \set{0,\ldots,3}$ must hold. Similarly, for every graph $H'_j\in \hset^B$ and vertex $y\in S(H'_j)$, let $k(y)$ be the total number of pairs in $\bigcup_{e=(v_i,v'_j)\in \delta_{\hat G}(v'_j)}M'_{i,j}$, in which vertex $y$ participates. Then $\sum_{y\in H'_j}k(y)=D(H'_j)$, and for every vertex $y\in S(H'_j)$, $k(y)\in \set{0,\ldots,3}$ must hold.
\end{lemma}

\begin{proof}
	We build the following directed flow network. We start with a bipartite graph $(X',Y',E'')$, with $X'=\bigcup_{i=1}^rS(H_i)$ and $Y'=\bigcup_{j=1}^{r'}S(H_j)$, and we let $E''=\bigcup_{e=(v_i,v'_j)\in E(\hat G)}M_{i,j}$. All edges are directed from $X'$ towards $Y'$, and they have capacity $2$ each. For all $1\leq i\leq r$, we add a vertex $s_i$, that connects to every vertex in $S(H_i)$ with an edge of capacity $3$. For all $1\leq j\leq r'$, we add a vertex $t_j$, to which every vertex of $S(H'_j)$ connects with an edge of capacity $3$. Lastly, we add a source vertex $s$, and a destination vertex $t$. For all $1\leq i\leq r$, we add an edge $(s,s_i)$ of capacity $D_i$, and for all $1\leq j\leq r'$, we add an edge $(t_j,t)$ of capacity $D_j$.
	
	We claim that this network as a valid $s$-$t$ flow of value $D$. We obtain this flow as follows. Consider an edge $e=(v_i,v'_j)$. Recall that we are given a weight $w_e\leq N^{h-j}$, and a matching $M_{i,j}$ of cardinality $\ceil{7N^{h-j}/8}$ between some vertices of $S(H_i)$ and some vertices of $S(H'_j)$. We send $\frac{8w(e)}{7N^{h-j}}$ flow units on every edge of $E_{i,j}$. Note that, since $w(e)\leq N^{h-j}$, the flow on every edge of $M_{i,j}$ is less than $2$, and the total flow sent on the edges of $M_{i,j}$ is $w(e)$.
	
	
	Consider any star $J\in \jset$. Assume w.l.o.g. that the center of the star is some vertex $v_i\in X$. From the above discussion, for every edge $(v_i,v'_j)$ of the star, for every pair of vertices $x\in S(H_i),y\in S(H'_j)$, at most two flow units are sent on edge $(x,y)$. Consider now some vertex $x\in S(H_i)$. We claim that the total flow that is sent to $x$ via all edges in $\bigcup_{(v_i,v'_j)\in E(J)}M'_{i,j}$ is also bounded by $2$. Indeed, we are guaranteed that $\sum_{e\in \delta_J(v_i)}w(e)\leq D(H_i)\leq |S(H_i)|\leq N^{h-j}$. For every superedge $e=(v_i,v_{j'})\in \delta_J(v_i)$, if there is an edge $(x,y)\in M_{i,j}$ with $y\in S(H'_j)$, then the amount of flow sent along this edge is $\frac{w(e)}{|M_{i,j}|}=\frac{w(e)}{\ceil{7N^{h-j}/8}}$. Therefore, the total amount of flow that vertex $x$ receives via matchings $M_{i,j}$ that correspond to edges $e=(v_i,v'_{j'})$ of the star $J$ is bounded by:
		
		\[\sum_{e\in \delta_J(v_i)} \frac{w(e)}{\ceil{7N^{h-j}/8}}\leq \frac 8 7.\]

Since every vertex of $\hat G$ participates in at most two stars in $\jset$, we conclude that so far every vertex of $X'$ sends less than three flow units, and every vertex of $Y'$ receives less than three flow units. 


For all $1\leq i\leq r$, for every vertex $x\in S(H_i)$, the amount of flow that we send on edge $(s_i,x)$ is equal to the amount of flow that currently leaves vertex $x$. From the definition of star covering, and from our definition of the flow so far, the total amount of flow leaving $s_i$ is precisely $D(H_i)$. We send $D(H_i)$ flow units via the edge $(s,s_i)$. Similarly, for all $1\leq j\leq r'$, for every vertex $y\in S(H'_j)$, the amount of flow that we send on edge $(y,t_j)$ is equal to the amount of flow that vertex $y$ currently recevies, which is at most $3$. The total amount of flow now entering vertex $t_j$ is precisely $D'(H'_j)$, and we send this amount of flow via the edge $(t_j,t)$. Overall we obtained a valid $s$-$t$ flow of value $D$ in this directed flow network. From the integrality of flow, there is an integral flow in this flow network of the same value. This integral flow defines a collection $\qset$ of paths. For every edge $(v_i,v'_{j'})\in E(\hat G)$, we denote by $M'_{i,j}$ the multiset of edges from $M_{i,j}$ that participate in the paths in $\qset$. 

For every graph $H_i\in \hset^A$ and vertex $x\in S(H_i)$, let $k(x)$ be the total number of pairs in $\bigcup_{e=(v_i,v'_j)\in \delta_{\hat G}(v_i)}M'_{i,j}$, in which vertex $x$ participates. From the discussion so far, and from the capacity constraints on the edges of the flow network,  $\sum_{x\in S(H_i)}k(x)=D(H_i)$ must hold, and moreover, for every vertex $x\in S(H_i)$, $k(x)\in \set{0,\ldots,3}$. Similarly, for every graph $H'_j\in \hset^B$ and vertex $y\in S(H'_j)$, let $k(y)$ be the total number of pairs in $\bigcup_{e=(v_i,v'_j)\in \delta_{\hat G}(v'_j)}M'_{i,j}$, in which vertex $y$ participates. Then $\sum_{y\in H'_j}k(y)=D(H'_j)$, and for every vertex $y\in S(H'_j)$, $k(y)\in \set{0,\ldots,3}$ must hold.
\end{proof}



\paragraph{Global Routing}
For every edge $e=(v_i,v'_j)\in E(\hat G)$, we consider the resulting collection $M'_{i,j}$ of pairs of vertices. We define a (multi)-set $\pset'(v_i,v'_j)\subseteq \pset(v_i,v_j')$ as follows. For every pair $(x,y)\in M'_{i,j}$ of vertices, we include in $\pset'(v_i,v'_j)$ the unique path $P(x,y)\in \pset(v_i,v_j')$ connecting $x$ to $y$ (if pair $(x,y)$ appears several times in $M'_{i,j}$, then we include the corresponding number of such pairs). Clearly, $|\pset'(v_i,v_j')|=|M'_{i,j}|$, the paths in $\pset'(v_i,v'_j)$ cause congestion at most $N^3$ in $H$, and each path has length at most $d'$.

Let $\qset^0=\bigcup_{(v_i,v'_j)\in E(\hat G)}\pset'(v_i,v'_j)$ (again, set $\qset^0$ is a multiset, so if some path appears several times in some set $\pset'(v_i,v'_j)$, then it will appear several times in $\qset^0$. Since $|\hset|=N$, the paths in $\qset^0$ cause congestion at most $N^5$, and each path has length at most $d'$ as before.

\subsection*{Step 4: Local Routing}


Consider some graph $H_i\in \hset^A$. We have defined a set $R_i\subseteq S(H_i)$ of $D_i$ vertices of $H_i$ that need to be routed. For every vertex $x\in S(H_i)$, we are also now given a value $k(x)\in \set{0,\ldots,3}$, which is exactly the number of paths in $\qset^0$ for which vertex $x$ serves as an endpoint. We are also guaranteed that $\sum_{x\in V(H_i)}k(x)=D_i$. We can then construct three sets $X_i^1,X_i^2,X_i^3$ of vertices of $S(X)$, such that for every vertex $x\in S(X)$, each of the three sets contains at most one copy of $x$; and the number of sets in $\set{X_i^1,X_i^2,X_i^3}$ containing $x$ is exactly $k(x)$. Clearly, $|X_i^1|+|X_i^2|+|X_i^3|=D_i$. We also partition the set $R_i$ of vertices into three subsets $R_i^1,R_i^2,R_i^3$ arbitrarily, so that, for all $1\leq a\leq 3$, $|R_i^a|=|X_i^a|$. Since $R_i\subseteq S(H_i)$, from the properties of level-$(j+1)$ structure, for each $1\leq a\leq 3$, there is a set $\hat\qset_i^a$ of $|X_i^a|$ paths in graph $H_i$, routing every vertex of $R_i^a$ to a distinct vertex of $X_i^a$, such that the length of every path is at most $d''_{j+1}$, and the paths cause congestion at mot $\eta'_{j+1}$ in graph $H_i$. 
Let $\hat \qset_i=\bigcup_{a=1}^3\hat \qset_i^a$. Notice that the paths in $\hat \qset_i$ route every vertex of $R_i$ to some vertex of $S(H_i)$, such that, for every vertex $x\in S(H_i)$, exactly $k(x)$ paths of $\hat \qset_i$ terminate at $x$. The paths in $\hat \qset_i$ cause congestion at most $3\eta'_{j+1}$ in graph $H_i$, and have length at most $d''_{j+1}$ each.

By exploiting the embedding of graph $H_i$ into $G$, we obtain a collection $\qset_i$ of paths in graph $H$. As before, the paths of $\qset_i$  route every vertex of $R_i$ to some vertex of $S(H_i)$, such that, for every vertex $x\in S(H_i)$, exactly $k(x)$ paths of $ \qset_i$ terminate at $x$. The paths in $ \qset_i$ have length $d''_{j+1}\cdot d'$ each. We will analyze the congestion caused by all such sets of paths together, once we finish the construction of the local routing. We denote by $\qset^1=\bigcup_{i=1}^r\qset_i$.

We process graphs $H'_j\in \hset^B$ similarly. For each such graph, we construct a set $\hat \qset'_j$ of paths in $H'_j$, that route every vertex of $R'_j$ to some vertex of $S(H'_j)$. We ensure that for every vertex $x\in S(H'_j)$, exactly $k(x)$ paths of $\hat \qset'_j$ terminate at $x$. As before, the paths in  $\hat \qset'_j$ cause congestion at most $3\eta'_{j+1}$ in graph $H'_j$, and have length at most $d''_{j+1}$ each.

By exploiting the embedding of graph $H'_j$ into $G$, we obtain a collection $\qset'_j$ of paths in graph $H$. As before, the paths of $\qset'_j$  route every vertex of $R'_j$ to some vertex of $S(H'_j)$, such that, for every vertex $x\in S(H'_j)$, exactly $k(x)$ paths of $ \qset'_j$ terminate at $x$. The paths in $ \qset'_j$ have length  $d''_{j+1}\cdot d'$ each. We denote by $\qset^2=\bigcup_{j=1}^{r'}\qset'_j$.


Consider now the set $\qset$ of paths that is obtained by concatenating the paths in $\qset^1,\qset^0$, and $\qset^2$. Then the paths in $\qset^1$ route every vertex of $\hat A=\bigcup_{i=1}^rR_i$ to a distinct vertex of $\hat B=\bigcup_{j=1}^{r'}R'_j$. The length of every path is at most $2d''_{j+1}\cdot d'+d'\leq 3d''_{j+1}\cdot d'$. We now analyze the total congestion caused by the paths in $\qset$.

The paths in $\qset^0$ cause congestion at most $N^5$ in $H$. For all $1\leq i\leq r$, the paths in $\hat \qset_i$ cause congestion at most $3\eta'_{j+1}$ in graph $H_i$, and  for all $1\leq i'\leq r'$, the paths in $\hat \qset_{i'}$ cause congestion at most $3\eta'_{j+1}$ in graph $H'_j$. Note that our embedding of graph $\left (\bigcup_{i=1}^rH_i\right )\cup \left  (\bigcup_{i'=1}^{r'}H'_{i'}\right )$ has congestion $\eta_j=N^{6\eps'/\eps}\cdot (x_{j+1})^2$ (where $x_j\leq N^{O(\eps'/\eps^2)})$ always holds). So can bound $\eta_j\leq N^{O(\eps'/\eps^2)}$. So we get total congestion due to paths in $\qset$ bounded by $N^5+3\eta'_{j+1}\cdot N^{O(\eps'/\eps^2)}$.


Final bound: can set $\eta'_h=N^5$, and $\eta'_j=\eta'_{j+1}\cdot N^{c\eps'/\eps^2}$. This will mean that $\eta'_0\leq N^{5+c\eps'/\eps^2}\leq N^6$ if $c\eps'<\eps^2$. Also $d''_j\leq 3d''_{j+1}\cdot d'$.
@@@


\mynote{can't use index $j$ because it's the level index. Switch to $i'$? also need to define $R_i$ and $R'_{i'}$. Add to prelims a claim about having a set of paths in $H$, embedding of $H$ into $G$, and resulting set of paths in $G$; path lengths and congestion.}

